FlexConv: Continuous Kernel Convolutions with Differentiable Kernel Sizes

When designing Convolutional Neural Networks (CNNs), one must select the size\break of the convolutional kernels before training. Recent works show CNNs benefit from different kernel sizes at different layers, but exploring all possible combinations is unfeasible in practice. A more efficient approach is to learn the kernel size during training. However, existing works that learn the kernel size have a limited bandwidth. These approaches scale kernels by dilation, and thus the detail they can describe is limited. In this work, we propose FlexConv, a novel convolutional operation with which high bandwidth convolutional kernels of learnable kernel size can be learned at a fixed parameter cost. FlexNets model long-term dependencies without the use of pooling, achieve state-of-the-art performance on several sequential datasets, outperform recent works with learned kernel sizes, and are competitive with much deeper ResNets on image benchmark datasets. Additionally, FlexNets can be deployed at higher resolutions than those seen during training. To avoid aliasing, we propose a novel kernel parameterization with which the frequency of the kernels can be analytically controlled. Our novel kernel parameterization shows higher descriptive power and faster convergence speed than existing parameterizations. This leads to important improvements in classification accuracy.

==> tables/appx-classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions?}}
\label{tab:full-smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN \citep{chang2017dilated} & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN \citep{li2018independently} & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN \citep{bai2018empirical} &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM \citep{trinh2018learning} & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. \citep{trinh2018learning} &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet \citep{bai2018trellis}& 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM \citep{gu2020improving} & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout \citep{gu2020improving} & - & 99.27 & 96.51 & \textbf{74.40} & - \\
  HiPPO \citep{gu2020hippo} & 0.5\sc{m} & - & \textbf{98.30} & - & - \\
  Lipschitz RNN \citep{erichson2020lipschitz} & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN \citep{rusch2020coupled} & 134\sc{k} & \textbf{99.4} & 97.3 & - & 59.0 \\
  UnICORNN \citep{rusch2021unicornn} & 135\sc{k} & - & 98.4 & - & \textbf{62.4} \\
  pLMU \citep{chilkuri2021parallelizing} & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & \todo{...\sc{m}} & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & \todo{...\sc{m}} & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & \textbf{99.55} &\textbf{ 98.57} & \textbf{74.58} & \textbf{67.37} \\
\midrule
FlexTCN-2 & 108\sc{k} & \textbf{99.60} & \textbf{98.61} & \textbf{78.99} &  \textbf{67.11}\\
FlexTCN-4 &  241\sc{k} & \textbf{99.60} & \textbf{98.72} & \textbf{80.26} & \textbf{67.42}\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 & \todo{...\sc{m}} & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & \todo{...\sc{m}} & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & \todo{...\sc{m}} &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

==> tables/classification-1d.tex <==
\begin{table}
\centering
\vskip -2mm
\caption{Test accuracy on sMNIST, pMNIST, sCIFAR10 and npCIFAR10. \todo{Conclusions.} \todo{Select models \& ablations to keep.} Tab.~\ref{tab:full-smnist} shows more results, including more baselines and ablations.}
\label{tab:smnist}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{cccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{sMNIST} & \sc{pMNIST} & \sc{sCIFAR10} & \sc{npCIFAR10} \\
 \midrule
 DilRNN & 44\sc{k} & 98.0 & 96.1 & - & -\\
  IndRNN & 83\sc{k} & 99.0 & 96.0& - & - \\
  %LSTM \citep{bai2018empirical} &70\sc{k}& 87.2 & 85.7  & - \\
 %GRU \citep{bai2018empirical} &70\sc{k}&   96.2 & 87.3  & - \\
   TCN &70\sc{k}& 99.0 & 97.2  & - & - \\
  r-LSTM & 0.5\sc{m} & 98.4 & 95.2 & 72.2 & -\\
 Self-Att. &0.5\sc{m} & 98.9 & 97.9 & 62.2 & -\\
 TrellisNet & 8\sc{m} & 99.20 & 98.13 & 73.42 & - \\
 URLSTM & - & 99.28 & 96.96 & 71.00 & - \\
  URGRU + Zoneout  & - & 99.27 & 96.51 & 74.40 & - \\
  HiPPO & 0.5\sc{m} & - & 98.30 & - & - \\
  Lipschitz RNN & 158\sc{k} & 99.4 & 97.3 & 64.2 & 59.0 \\
  coRNN & 134\sc{k} & 99.4 & 97.3 & - & 59.0 \\
  UnICORNN & 135\sc{k} & - & 98.4 & - & 62.4 \\
  pLMU  & 165\sc{k} & - & 98.49 & - & -\\
\midrule
CKCNN-2 & 98\sc{k} & 99.31 & 98.00 & 62.25 & 60.5\\
CKCNN-2-Big & 1\sc{m} & 99.32 & 98.54 & 63.74 & 62.2 \\
CKTCN$_{\text{\sc{Fourier}}}$-2 & & 99.44 & 98.40 & 68.28 & 66.26 \\
CKTCN$_{\text{\sc{Gabor}}}$-2 & & 99.52 & 98.38 & 69.26 & 67.52 \\
CKTCN$_{\text{\sc{MAGNet}}}$-2 & 105\sc{k} & 99.55 & 98.57 & 74.58 & 67.37 \\
\midrule
FlexTCN-2 & 108\sc{k} & 99.60 & 98.61 & 78.99 & 67.11\\
FlexTCN-4 &  241\sc{k} & 99.60 & \textbf{98.72} & 80.26 & 67.42\\
FlexTCN-6 & 375\sc{k} & \textbf{99.62} &  98.63 & \textbf{80.82} & \textbf{69.87} \\
\midrule
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & 99.03 & 95.36 & 69.24 & 57.27 \\
FlexTCN$_{\text{Fourier}}$-6 & & 99.49 & 97.97 & 74.79 & 67.35 \\
FlexTCN$_{\text{Gabor}}$-6 & &  99.50 & 98.37 & 78.36 & 67.56 \\
FlexTCN$_{\text{MAGNet}}$-6 & 375\sc{k} & \textbf{99.62} &  \textbf{98.63} & \textbf{80.82} & \textbf{69.87} \\
\bottomrule
\end{tabular}}
\end{small}
\end{table}

% DilRNN \citep{chang2017dilated}, 
% IndRNN \citep{li2018independently}, 
% TCN \citep{bai2018empirical}, 
% r-LSTM \citep{trinh2018learning}, 
% Self-Att. \citep{trinh2018learning}, 
% TrellisNet \citep{bai2018trellis}, 
% URLSTM \citep{gu2020improving}, 
% URGRU + Zoneout \citep{gu2020improving}, 
% HiPPO \citep{gu2020hippo}, 
% Lipschitz RNN \citep{erichson2020lipschitz}, 
% coRNN \citep{rusch2020coupled}, 
% UnICORNN \citep{rusch2021unicornn} and
% pLMU \citep{chilkuri2021parallelizing}.

==> tables/classification-cifar10.tex <==
\begin{table}
% \begin{wraptable}{r}{0.45\textwidth}
\vspace{-0mm}
\centering
\caption{Results on CIFAR-10. FlexNet is competitive with CIFARResNets and other learnable kernel size works. The FlexConv mask and MAGNet both improve over the baseline CKConv methods. We report results over three runs per setting. Time is reported as seconds per epoch of a converged model. Tab.~\ref{tab:full-cifar-10} shows more results, including more ablations. *Results are taken from the respective original works instead of reproduced. \!\dagger Results are from single run.}
\label{tab:cifar-10}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \sc{CIFAR-10} & \multirow{2}{*}{\sc{Time}} \\
    & & \sc{Acc.} & \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 92.9*\!\dagger & - \\ \midrule
    DCN-$\sigma^{ji}$ & 0.47\sc{m} & 89.7 $\pm$ 0.3* & - \\
    N-Jet-CIFARResNet32 & 0.52\sc{m} & 92.3 $\pm$ 0.3* & - \\
    N-Jet-ALLCNN & 1.07\sc{m} & 92.5 $\pm$ 0.1* & - \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 89.5 $\pm$ 0.3 & 41s   \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 78.0 $\pm$ 0.3 & 242s  \\
    FlexNet-7 w/ N-Jet & 0.70\sc{m} & 91.7 $\pm$ 0.1 & 409s  \\ \midrule
    % \midrule
    CKCNN-7 & 0.63\sc{m} & 71.7* & 266s \\ % 71.70
    CKCNN$_{\text{Gabor}}$-7 & 0.67\sc{m} & 87.6* & \todo{69s} \\ % 87.65
    CKCNN$_{\text{MAGNet}}$-7 & 0.67\sc{m} &  85.9* & 299s \\ % 85.91
    \midrule
    FlexNet$_{\text{SIREN}}$-7 & 0.63\sc{m} & 88.9* & 105s \\ % 88.88
    FlexNet$_{\text{Gabor}}$-7 & 0.67\sc{m} & 92.0* & 178s \\ % 91.99
    \midrule
    FlexNet-7 & 0.67\sc{m} & 92.2 $\pm$ 0.1 & 166s \\
 \bottomrule
\end{tabular}}
% \end{sc}
% \end{small}
\end{center}
\vspace{-7mm}
\end{table}
% \end{wraptable}

==> tables/classification-sequences.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\vspace{-5mm}
\vskip -2mm
\caption{Test accuracy on Character Trajectory, Speech Commands, Speech Commands Raw. \todo{Conclusions.}}
\label{tab:time-series}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccc}
\toprule
\sc{Model} & \sc{Size} & \sc{CT} & \sc{SC} & \sc{SC\_raw} \\
\midrule
GRU-ODE & 89\sc{k} & 96.2 & 44.8 & $\sim$10.0 \\
GRU-$\Delta t$ & 89\sc{k} & 97.8 & 20.0 & $\sim$10.0 \\
GRU-D & 89\sc{k} & 95.9 & 23.9 & $\sim$10.0 \\
ODE-RNN & 89\sc{k} & 97.1 & 93.2 & $\sim$10.0 \\
NCDE  & 89\sc{k} & 98.8 & 88.5 & $\sim$10.0 \\
\midrule
CKCNN & 100\sc{k} &\textbf{ 99.53 }& 95.27 & 71.66 \\
CKTCN$_{\text{Fourier}}$ & & - & 95.65 & 74.90 \\
CKTCN$_{\text{Gabor}}$ &  & - & 96.66 &  78.10 \\
CKTCN$_{\text{MAGNet}}$ & 105\sc{k} &  \textbf{99.53} & \textbf{97.01} & \textbf{80.69} \\
\midrule
FlexTCN-2 & 105\sc{sk} & \textbf{99.53} & \textbf{97.10} & \textbf{88.03}  \\
FlexTCN-4 & 239\sc{k} & \textbf{99.53} & \textbf{97.73} & \textbf{90.45}   \\
FlexTCN-6 & 373\sc{k} & \textbf{99.53} & \textbf{97.67} & \textbf{91.73} \\
\midrule
FlexTCN$_{\text{SIREN}}$-6 &  & - & 95.83 & \\
FlexTCN$_{\text{Fourier}}$-6 & & - & 97.62 &  \\
FlexTCN$_{\text{Gabor}}$-6 & & - & 97.35 & \\
FlexTCN$_{\text{MAGNet}}$-6 & 373\sc{k} & - & \textbf{97.67} & \textbf{91.73} \\
\bottomrule
\end{tabular}}
\end{small}
\vspace{5mm}
\end{wraptable}

==> tables/crossres-cifar10.tex <==
\begin{table}

\begin{minipage}{0.50\textwidth}
\vspace{8mm}
\centering
\caption{Results for alias-free FlexNets on \todo{CIFAR-10}.
% FlexNets reduce the accuracy gap at upscaling more than all other methods. We train each model for 100 epochs at resolution $16 \times 16$, then evaluate it at resolution $32 \times 32$. We report results over three runs per setting.
}
\label{tab:crossres}
\begin{center}
%\vskip -3mm
% \begin{small}
% \begin{sc}
\scalebox{0.7}{
\begin{tabular}{cccc}
\toprule
    \multirow{2}{*}{\sc{Model}} & \multirow{2}{*}{\sc{Size}} & \multicolumn{2}{c}{\sc{CIFAR-10 Acc.}} \\
    & & 16 px & $\Delta_{16 \textrm{px}}$ 32 px \\ \midrule % & fine-tuned \\ \midrule
    CIFARResNet-44 & 0.66\sc{m} & 85.8 $\pm$ 0.2 & -31.6 $\pm$ 1.3 \\ \midrule
    % 85.4 $\pm$ 0.3 & -31.2 $\pm$ 2.8 \\ \midrule % & 92.6 $\pm$ 0.2 \\ \midrule
    FlexNet-7 w/ conv. ($k = 3$) & 0.17\sc{m} & 85.3 $\pm$ 0.2 & -21.2 $\pm$ 1.0 \\ % & \textbf{90.1} $\pm$ 0.1  \\
    FlexNet-7 w/ conv. ($k = 33$) & 20.0\sc{m} & 67.7 $\pm$ 0.6 & -57.1 $\pm$ 1.6 \\ % & 79.2 $\pm$ 0.4  \\
    FlexNet-7 w/ N-Jets & 0.70\sc{m} & \textbf{86.4} $\pm$ 0.2 & -5.5 $\pm$ 1.3 \\ \midrule % & 89.5 $\pm$ 0.1  \\ \midrule
    CKCNN-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 45.9 $\pm$ 1.0 & -15.8 $\pm$ 1.2 \\
    FlexNet-7$_{\textrm{SIREN}}$ & 0.63\sc{m} & 70.4 $\pm$ 0.8 & -50.0 $\pm$ 16.9 \\ \midrule
    FlexNet-7 w/o reg. & 0.67\sc{m} & \textbf{86.4} $\pm$ 0.4 & -34.4 $\pm$ 14.3 \\ \midrule % & 88.8 $\pm$ 0.6 \\ \midrule
    FlexNet-7 w/ reg. $f^+_{\textrm{MAGNet}}$ & 0.67\sc{m} & \textbf{86.5} $\pm$ 0.1 & -3.8 $\pm$ 2.0 \\ % & 89.0 $\pm$ 0.3  \\
    FlexNet-7 w/ reg. $f^+_{\textrm{FlexConv}}$ & 0.67\sc{m} & 85.1 $\pm$ 0.3 & \textbf{-3.3} $\pm$ 0.3 \\ % & 87.6 $\pm$ 0.2 \\
 \bottomrule
\end{tabular}}
\end{center}
% \vspace{-5mm}
\end{minipage}\hspace{5mm}
\end{table}
